Architectural Support for Software Performance in Continuous Software Engineering: A Systematic Mapping Study

The continuous software engineering paradigm is gaining popularity in modern development practices, where the interleaving of design and runtime activities is induced by the continuous evolution of software systems. In this context, performance assessment is not easy, but recent studies have shown that architectural models evolving with the software can support this goal. In this paper, we present a mapping study aimed at classifying existing scientific contributions that deal with the architectural support for performance-targeted continuous software engineering. We have applied the systematic mapping methodology to an initial set of 215 potentially relevant papers and selected 66 primary studies that we have analyzed to characterize and classify the current state of research. This classification helps to focus on the main aspects that are being considered in this domain and, mostly, on the emerging findings and implications for future research

==> _discussion_merged_with_results_.tex <==
\section{Discussion}
\label{sec:discussion}
\noindent
In this section, we will discuss the results obtained outlining some implications for researchers and practitioners working in the performance engineering, and DevOps domain. 
Although the DevOps domain is relatively young compared to performance engineering, significant contributions have been published in the last ten years and researchers are becoming more and more active (Figure~\ref{fig:pubs_by_year}).

\AN{La crescente complessità dei sistemi software (da intendere sia verticalmente ossia che poggiano su stack complessi, sia orizzontalmente perchè integrano component hw/sw sempre più eterogenee) richiede un uso oculato delle risorse anche in vista delle politiche richieste di riduzione degli impatti ambientali diretti e indiretti  in linea col principio del “non arrecare danni significativi” all’ambiente (“do no significant harm” – DNSH) che ispira il NGEU (Next Generation EU).}

\AN{Inoltre la necessità di apportare modifiche a sistemi software che governano la vita personale (domotica e ehealth, servizi per i servizi alla famiglia e ai diritti fondamentali quali istruzione, sanità e sicurezza delle persone, le aziende e le istituzioni, è sempre crescente spingentosi nel continuo. Questa velocità sacrifica la qualità del software riducendo la fase di V\&V, quindi anche questa V&V deve essere spostata nel continuo per catturare deviazione sui requisiti di qualità (continuo monitoring) e sviluppo di tecniche e metodologie (dalla riprogettazione architetturale alla codifica di meccanismi di basso livello) che possano migliorare la qualità del sistema in continua evoluzione.}

\AN{La self-adaptive non è più sufficiente perchè la self-adaptive codifica meccanismi e strategie di adattamento a risposta di problemi osservati durante la verifica e validazione. Nel mondo continuos, sacrificando questa fase, vanno identificate e definite metodologie continous che considerino anche questi aspetti.}

\AN{Tutto ciò premesso, in questo paper ci siamo concentrati sul continous software performance engineering, per la gestione delle risorse e per garantire idonei tempi di risposta di sistemi aperti e integrati, considerando chiave la vista architetturale che ne semplifica la trattazione.}



\subsection{RQ$_1$: What research areas and domains have been investigated?}
\label{sec:discussion:rq1}
\noindent
\emph{Software performance engineering} and/or \emph{Software architecture} are the research areas where all papers are positioned; most of them are related to at least one of the continuous dimensions (introduced in Section \ref{sec:related}). In particular, a large number of papers proposes continuous monitoring of data to realize continuous development, delivery or integration that improve performance in software architectures; this is justified by the fact that the monitored data enables performance analysis. Such a result confirms that, in the areas of software architecture and software performance, continuous software engineering is an emergent topic that is progressively affecting researchers and practitioners.
%
On the other hand, our results show that a small number of selected papers cover the \emph{DevOps} and the \emph{Agile} development processes. This unveiling an interesting gap to be filled by the research community, despite the existing conferences and systematic reviews on the topic suggest that software engineering researchers have a strong interest in the topic.
%
%For each area, the relationship between \emph{fully} and \emph{partially investigated} areas
%is proportional (i.e., a good percentage of the areas are fully investigated). 
%
Even if a large number of selected papers has been fully identified as in the \emph{Continuous software engineering} area, the number of papers that partially investigates this area increases. Beyond that, several selected papers have not been placed within a context of \emph{Continuous software engineering} or \emph{DevOps}. This can be attributed to the fact that these works do not explicitly place themselves in these areas, even if they actually offer solutions that cover several aspects of an iterative development process where updates are made continuously. This confirms that this emerging theme that is gaining ground.


With respect to the considered domains, \emph{Component-based software/SOA/Microservices} and \emph{Complex software systems} are mostly investigated. These domains are characterized by the existence of different components, services or subsystems. These can be independent of each other (e.g., microservices) or have strong dependencies and relationships between them (and the environment), as in many complex systems. In both cases, however, the presence of heterogeneous components makes it necessary to integrate these activities in a continuous development and maintenance (e.g., DevOps).
The component-based development paradigm is based on the concept of reuse within distinct services, enabling integration. Once integrated and implemented, these services need to enter a continuous dimension; i.e., to know and analyze the behavior after the integration and not only of the single service / component, therefore also important in a performance context.

Next, the results show the domains of \emph{Cloud} and \emph{Distributed systems}, characterized by stack and infrastructure complexity. For example, if a cloud system is not natively designed from a performance standpoint, it can generate hysterical behavior. This is typical in open systems, with uncontrolled requests; it follows that during the integration and evolution of these systems, continuous development can identify the occurrence of further problems not observed before.

While a greater presence of the previous domains is justified by their nature, the following domains are less investigated; this result is probably linked to the fact that these are more recent and innovative domains not yet widely investigated, for instance in the case of \emph{Data intensive systems} where the maximum use of big data and ML requires an efficient management of resources.


%\RE{I domini più investigati sono CBS/SOA/Microservices e Complex software systems. Quesueti domini sono caratterizzati dall'esistenza di diverse componenti, servizi o subsysterms. Tali parti possono essere indipendenti tra loro (e.g., microservices)o ci possono essere dependencies and relationships between their parts (and the environment), come in molti systemi complessi. In entrabe i casi però, la presenza di componenti etereogenee rende naturale l'esigenza di integrate these activities in a development and maintenance continuum (eg, DevOps). usi un ocmponent bbased perchè per il paradigma li riusi nei servii integrandoli, il servizio integrato richiede che quando integri e iniia ad operare hai bisogno di un ocntinouous (deve conoscere le parti anche nell'integrazione non nel singolo), quindi importante anche performance.}

%\RE{Integration testing ti verifica se le componenti integrate funzionano bene, se il sitema nel complesso funziona bene, fai  testing, anche solo una componente può creare un malfunzionamento.}

%\RE{Poi ci sono i cloud e distribbuted abbbiamo uan complessità di stack, di infrastreuttura. Nativamente il cloud forns eo cloud non è porgettato bene dal punto di vista delle performance può generare un comportamento isterico. sistema aperto che ha richeista incontrollate, quindi quando integro nello  sviluppo continuo possono manifestarsi ulteriori problemi non osservati prima.}

%\RE{se ho uno sviluppo agile ma non ho un continuo non rieeco a fare analisi di pari passo.}

%\RE{data intensive è nuovo e porta stress sulle risorse, ML super usato }
%
%\RE{CPS, real-time, domini innovativi su cui è richiesta una tempestività di risposta}
%
%\RE{verificare se real-time è in contribution self-adaptive. }

%We can observe that application domains close to software systems (e.g., \emph{Microservices}) have garnered attention from the research community, whereas there is a lack in the research coverage in all application domains that combine software with physical systems such as embedded systems, CPS, and real-time systems. Surprisingly, \emph{Cloud} application domain is little considered in the considered topic.
 
 
 
%\RE{DISCUSSION: manca una considerazione che lega i domini alle diverse discipline (vedi venue), o anche una considerazione sul fatto che spesso il dominio è molto generale e non specifico (fatta eccezione per microservices e cloud) }






\subsection{RQ$_2$: What and how performance problems have been addressed?}
\label{sec:discussion:rq2}
\noindent
Most of the work in this area is aimed at solving \emph{Performance evaluation and assessment} problems. This is a relevant goal in the development of modern systems, where increasingly agile paradigms require that performance analyzes be in a continuous dimension in order to be effective.

It's interesting that 21 papers aim to provide \emph{Quality of service}. 

%Our results show that most of the selected papers deal with \emph{Performance evaluation and assessment} 
A smaller number of works address \emph{Uncertainty} and \emph{Resource allocation}, both of them are related to the requirements of the increased complexity of model systems (that are open, distributed and heterogeneous). 
Than can be seen as an emerging topic. 





More than half of these problems have been addressed through the support of tools and are well partitioned between \emph{Performance prediction}, \emph{Performance analysis} and \emph{Performance modelling}. Other ones are dedicated to \emph{Self-adaptation} approaches or, to a lesser extent, to providing \emph{Domain Specific Language}s. 

\RE{non hai continuous senza tools, pochi DSL (che vogliono fare un'astrazione per controllare la specifica, quindi lavori con tanti dati monitoring ma non alzi il livello di astrazione, forse siamo ancorati a un babsso livello. come si mappa uncertainty con DSL? )}


%\DT{la parte sotto e' collegata a RQ4}
Instead, we can see that \emph{Continuous engineering framework}s are not largely covered. This points out a gap between the emerged need in continuous engineering and the solutions provided.


\subsection{RQ$_3$: What instruments have been adopted?}
\label{sec:discussion:rq3}
\noindent
We have analyzed the selected papers under the vision that an approach can be classified as: \emph{input data} $\rightarrow$ \emph{methodology/technique} $\rightarrow$ \emph{output measures/indices}. Of course, not all selected papers clearly undergo this schema, but the obtained results provide some interesting insights about the combination frequencies of these three elements. Based on a straightforward observation of results, the highest focus (up today) has been given to \emph{performance modeling} and \emph{analysis} techniques that takes as input \emph{runtime/monitored} data and produce \emph{response time} and \emph{utilization} indices as output. This is a relevant confirmation of what is expected performance analysts should do in the context of continuous software engineering processes. It was, instead, unexpected that, no matter what is the technique adopted, quite rarely \emph{requirements} and \emph{data analytics} enter the process to target \emph{memory} and \emph{network bandwidth}. Indeed, this highlights a lack of investigation that, especially in the domain of distributed heterogeneous software systems, shall be crucial. Indeed, on one side, data analytics are ever more available and performance requirements are ever more stringent and, on another side, traditional performance measures (such as response time and utilization) in isolation do not provide an integrated vision of the system behavior, which could suffer by performance degradation due to a bad usage of memory and network connection.

% \VC{le discussions di RQ2 e RQ3 appaiono differenti dalle altre due?}

\subsection{RQ$_4$: What are the current research gaps?}
\label{sec:discussion:rq4}
%perchè ci sono questi gap? 
%perchè nessuno non lo ha fatto oppure manca una tecnica o ci sono degli impedimenti nello studiare qualcosa. dati, tools e tecniche sono disponibili per fare l'investigazione? ci sono incompatibiblità o un'area in cui c'è gap non ha senso per CSE.
\noindent
As it is evident from the results reported in Section~\ref{sec:results:rq4}, there is a noticeable difference in coverage among more established and emerging research topics.
The more general \emph{Performance evaluation} topic is a clear example of this.
It is among the most investigated topics in our study, not only because t is understandably at the center of our inquire, but probably because it is a very well established research topic  with a history spanning decades.

Nonetheless, when the same topic is combined with more recent trends of the software industry, like Agile and DevOps, it clearly lags behind in the number of paper covering it.
Apart from the obvious reason that more recent topics will probably receive less coverage in research, a more compelling justification could be found in the specific characteristics of Agile processes and practices.
In fact, Agile cycles are usually quite short on time as the main focus of such cycles is probably the fast release of new features.
While some tests, like acceptance test from the product owner, are understandably required before releasing a new feature, performance tests are usually not, as they are often very demanding on time and resources.
A possible solution might be to classify new requirements with low and high performance priority, and contemplate dedicating a considerate budget to performance analysis and testing.

Along the same line, specific needs of cloud-native systems not always align with the requirements of performance evaluation.
Most of the cloud-native systems are adopting continuous tracing tools (e.g., Jaeger, OpenTelemetry, AppDynamics) that allow to record execution traces withing highly distributed and dynamic environments.
Such tools might allow conducting some performance analysis as they usually provide additional information that is relevant to performance, such as the execution time of remote calls.
However, most companies are not experienced in conducting performance analysis on distributed traces, or do not prioritize performance aspects until they undermine user experience.

Differently from Agile, DevOps, and Cloud, the topic of uncertainty in software engineering has been relevant for quite some time.
Even so, it still represents an emerging topic in research, especially when considering performance evaluation in uncertain settings.
Evaluating performance while keeping uncertainty is an inherently difficult task.
The characteristics of software systems are getting  more dynamic due to many factors: they are more distributed because they are moving on the cloud or are composed by third parties software, they are open to a wider group of users, and, more importantly, they are expected to provide quality of service guarantees in ever-changing environments. 
In this context, performance evaluation has to deal with fluctuating workloads and great variability in resource demands, posing more challenges on the accuracy and validity over time of the prediction and analysis of performance results.
To deal with this problem, researchers started to study software performance under uncertainty, and our study finds that this is a research area not yet sufficiently investigated, but that might have great growing potential.

%Cosa e' stato gia' investigato e perche'
%\begin{itemize}
%    \item Performance evaluation. Reason: long history, ... 
%\end{itemize}
%
%
%Cosa e' stato investigato "poco" o per niente
%\begin{itemize}
%    \item Performance evaluation in Agile. Possible Reason: Lack of time. We believe that in Agile cycles are too short to perform performance testing, agile focuses mainly on providing new features instead of deeply test them. In particular, in agile, devs. focus on acceptance tests from product owner, that often do not include performance test. A possible solution might be to classify new requirements with low and high performance priority, and consider performance analysis and testing. 
%    
%    \item Performance in cloud-native systems. Most of the cloud-native systems are adopting continuous tracing tools (Jaeger, OpenTelemetry, AppDynamics..). These tools might allow to conduct performance engineering experiments (or test). However, most of the companies are not experienced or do not consider/prioritize performance aspects.  
%
%    \item Uncertainty. The characteristics of the systems are getting  more dynamic due to many factors:
%    they are more distributed because they are moving on the cloud or are composed by third parties software; they are open to a wider group of users. 
%    Hence the fluctuating workload and the heavy usage of connections (even with mobile devices) with unstable characteristics pose more challenges on the accuracy and validity over time of the prediction and analysis of the system's performance. To deal with this problem, researchers started to study system's performance under uncertainty.    
%    
%    \item c'e' qualcosa che non e' stato investigato perche' mancano tools o tecniche? questo potrebbe esere un buon suggerimento per i lettori
%    \item c'e' qualcosa che non e' stato investigato perche' magari non ha senso farlo (e perche' non avrebbe senso?) 
%\end{itemize}




\subsection{Implications for practitioners and researchers}

\noindent
Practitioners can benefit of our results to understand how to apply software performance engineering for architectural support in the CSE/DevOps context, and which tool support is available.  Moreover they can benefit of the classification of methodologies applicable for architectural support for performance engineering in the context of continuous software development. Moreover, practitioners can understand if they are applying cutting edge technologies in the context of performance assessment in continuous software engineering or if there is room for updating the practices they are using.  

Researchers can benefit of our results to understand research trends, research gaps, and to better focus their future works. In particular, the software performance community can leverage this work to understand if their approaches are applicable in a CSE/DevOps context. Moreover, this study helps them to define the requirements that should drive the development of their tools, so as to increase the chances of industrial adoption.
Whereas, researchers in the field of CSE/DevOps can understand which methodologies and techniques can help them to improve the software performance at some stage in the development cycle. 




==> _old_results-RQ2.tex <==
\subsection{Research focus, coverage and maturity (RQ2)}%
\noindent
The RQ2 is related to research focus that we analyse discussing the results of our mapping study, and to research coverage and maturity. 
As described in Sect. \ref{sec:method-4}, the classification schema defines four main categories related to RQ2: Research area, Application domain, Target problem and Research contribution. In the following, we first discuss about the research focus and then we report on the research coverage and maturity. 

\vspace{0.2cm}
\subsubsection{Research focus}
\noindent
Fig.s~\ref{fig:classification_research_area}~--~\ref{fig:classification_research_contribution} depict the results of our mapping study for each of the above mentioned categories, by reporting the number of primary studies classified with respect to each keyword. We also show the variation of this mapping over the years, as reported in Fig. \ref{fig:rq2_mapping_in_time_avg}. Then, in order to deeply analyze the research focus, we also introduce two additional metrics that we call \emph{Scope} and \emph{Sharpness}.

\underline{\emph{Research area}}  (see Fig.~\ref{fig:classification_research_area}) describes the principal area of interest in which the primary studies contribute to (note that, each study may contribute to more than one area). As expected, primary studies mainly focus on the areas of \emph{Performance engineering} and \emph{Software architecture}, which is in line with the executed query. A significant attention is also given to \emph{Self-adaptation} approaches, that are capable of modifying system runtime behavior in order to achieve system objectives and goals. Many studies contribute to the areas of \emph{Continuous software engineering} and \emph{Continuous monitoring}, meaning that a large number of papers proposes continuous observation of data to realize continuous development/delivery/integration 
that improve performance in software architectures. This suggests that performance-targeted continuous software engineering is an emergent context that is progressively affecting researchers and practitioners.
Surprisingly, only few of the primary studies cover \emph{DevOps} and only 5 papers deal with architectural support of performance engineering in \emph{Agile} development process, unveiling interesting gap to be filled by the research community.

\begin{figure}[htpb]
    \centering
    \includegraphics[width=.98\linewidth]{figures/research_area_0.5_to_1.pdf}
    \caption{Research area.}%
    \label{fig:classification_research_area}
\end{figure}

\underline{\emph{Application domain}} (see Fig.~\ref{fig:calssification_domain}) covers specific field of application.  The main focus is on \emph{Complex software systems} (e.g., software-intensive systems in  telecommunications, industrial control, or business process management). Moreover, a significant number of applications is on \emph{Component-based Systems (CBS), Services (SOA) and Microservices}  technologies, while few of them cover \emph{Embedded systems}, \emph{Cyber Physical Systems (CPS)}, \emph{Real-time Systems} and \emph{Cloud}. A new emerging application domain is appearing that is related to big data and its management and analysis (i.e., \emph{Data intensive systems}).
We can observe that application domains close to software systems (e.g., Microservices) have garnered attention from the research community; whereas there is a lack in the research coverage in all application domains that combine software with physical systems such as embedded systems, CPS, and real-time systems. Surprisingly, Cloud application domain is little considered in architecture-supported performance-targeted continuous software engineering.


\begin{figure}[htpb]
    \centering
    \includegraphics[width=.98\linewidth]{figures/domain__systems_domain_0.5_to_1.pdf}
    \caption{Application domain.}%
    \label{fig:calssification_domain}
\end{figure}

\underline{\emph{Target problem}} (in Fig.~\ref{fig:classification_target_problem}) deals with the problems targeted by the primary studies. The obtained results confirm that most of the primary studies ($70\%$) concern to \emph{Performance evaluation}. $26\%$ of the primary studies cover the \emph{Quality of service}, and $18.5\%$ of them deals with \emph{Resource allocation}. This is an expected outcome that is strictly related to our query. Interestingly, the mapping unveils that  \emph{Uncertainty} and \emph{Performance requirement} are emerging as target problems. 

\begin{figure}[htpb]
    \centering
    \includegraphics[width=.98\linewidth]{figures/target_problem_0.5_to_1.pdf}
    \caption{Target problem.}%
    \label{fig:classification_target_problem}
\end{figure}

\underline{\emph{Research contributions}} (see Fig.~\ref{fig:classification_research_contribution}). From our analysis, we can state that most of the studies contribute to the research domain with \emph{Performance analysis, Performance modelling, and Performance prediction} approaches. Also, a considerable number of approaches propose a \emph{Continuous engineering framework}. Finally, a high number of studies (i.e., $29$) provides a \emph{Tool support} to aid performance engineering research. Interestingly, a new research contribution is emerging that is related to \emph{Domain Specific Languages} for which we report only $6$ primary studies over $54$ considered.

\begin{figure}[htpb]
    \centering
    \includegraphics[width=.95\linewidth]{figures/research_contribution_0.5_to_1.pdf}
    \caption{Research contribution}%
    \label{fig:classification_research_contribution}
\end{figure}

Fig.~\ref{fig:mapping_in_time_research_area_avg} shows that emerging research areas like \emph{Continuous software engineering} and \emph{DevOps} tend to attract more interest than, for instance, consolidated areas like Self-adaptation. Similar remarks can be done for the Fig.~\ref{fig:mapping_in_time_domain_avg}, where application domain like \emph{Cloud} and \emph{Data intensive systems} confirm the recent trend in the field. Among the target problems, \emph{Uncertainty} has been  employed only after 2015. Finally, Fig.~\ref{fig:mapping_in_time_contribution_avg} shows some interesting results. In fact, it seems that \emph{Performance analysis} and \emph{Self-adaptation} met with less interest respect to other types of contribution, like \emph{Continuous engineering framework} and \emph{Performance modelling} approaches. Fig.~\ref{fig:mapping_in_time_contribution_avg} confirms that \emph{Domain specific language} in the our research field is an emerging contribution.



\underline{\emph{Scope and Sharpness.}} 
As already said, in order to deeply analyze the Research focus, we introduced the following additional metrics: 
\begin{itemize}
    \item \emph{Scope}: it measures how intensely the selected primary studies cover the 26 keywords considered for RQ2. For each paper, we calculated the sum of the values we assigned to every keyword, thus obtaining $(0,26]$ as this metric range.
    \item \emph{Sharpness}: it measures how much the considered papers are sharp on our study context (i.e., with respect to the keywords considered for RQ2). It is calculated by counting the numbers of scores with value 1 (i.e., the keyword is fully covered) divided by 26 (i.e., number of keywords related to RQ2), thus obtaining $(0,1]$ as this metric range. 
\end{itemize}


In Fig.~\ref{fig:scope}, \emph{Scope} is represented by means of a histogram that shows its distribution vs. intervals of coverage metric. As expected, there are no papers with scope greater than 12 and only few cases greater than 10. In fact, the RQ2's keywords represent aspects that can hardly be addressed all simultaneously in one paper. On the other hand, we obtained few papers with scope less than 4, thus meaning that the identified keywords for category are representative enough of the mapping study context and goals. Such observations are confirmed also by the Gaussian trend of the distribution. 

\begin{figure}[htbp]
\centering
\subfloat[\label{fig:mapping_in_time_research_area_avg}Research area.]{
  \includegraphics[width=.95\linewidth]{figures/research_area_mapping_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:mapping_in_time_domain_avg}Application domain.]{
  \includegraphics[width=.95\linewidth]{figures/domain__systems_domain_mapping_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:mapping_in_time_target_problem_avg}Target problem.]{
  \includegraphics[width=.95\linewidth]{figures/target_problem_mapping_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:mapping_in_time_contribution_avg}Research contribution.]{
  \includegraphics[width=.95\linewidth]{figures/research_contribution_mapping_in_time_avg.pdf}
}
\caption{\label{fig:rq2_mapping_in_time_avg}Average variation of the mapping over the years (RQ2).}
\end{figure}



\begin{figure}[htbp]
\centering
\subfloat[\label{fig:scope}Scope]{
  \includegraphics[width=.95\linewidth]{figures/hist_Scope.pdf}
}
\hfil
\subfloat[\label{fig:sharpness}Sharpness]{
  \includegraphics[width=.95\linewidth]{figures/hist_Sharpness.pdf}
}
\caption{\label{fig:scope_sharpness}Scope and sharpness of primary studies}
\end{figure}


While this result means that most of the papers cover sufficiently well the aspects identified by the keywords, this does not give us information about how sharp on specific keywords they are. This analysis has been made through he \emph{Sharpness} metric (see Fig. \ref{fig:sharpness}), that considers only papers with some values equals to 1. The papers with the highest sharpness are those that focused well on our study context and goals (i.e., we evaluated that they fully cover one or more keywords). The papers with lower focus could marginally cover the keywords or be less focused on some specific aspects of RQ2's categories. 

\begin{figure}[htbp]
\centering
\subfloat[\label{fig:coverage_maturity_research_area}Research area]{
  \includegraphics[width=.95\linewidth]{figures/research_area_coverage_maturity.pdf}
}
\hfil
\subfloat[\label{fig:coverage_maturity_domain}Application domain]{
  \includegraphics[width=.95\linewidth]{figures/domain__systems_domain_coverage_maturity.pdf}
}
\hfil
\subfloat[\label{fig:coverage_maturity_target_problem}Target problem]{
  \includegraphics[width=.95\linewidth]{figures/target_problem_coverage_maturity.pdf}
}
\hfil
\subfloat[\label{fig:coverage_maturity_contribution}Research contribution]{
  \includegraphics[width=.95\linewidth]{figures/research_contribution_coverage_maturity.pdf}
}
\caption{\label{fig:coverage_maturity}Keywords coverage and maturity}
\end{figure}


There are no papers without specific sharpness, besides half of the papers are very focused on about 6 keywords (i.e., sharpness between 0,20 and 0,25). These results allow us to assume that a high number of existing approaches that fall within this context provides a sharp contribution to the relevant keywords here considered. 

\vspace{0.2cm}
\subsubsection{Research coverage and maturity}
\noindent
As final aspect for answering RQ2, we intend to assess the coverage and the maturity of the considered categories. In order to analyse this, we have defined other two metrics that specialize the previous described results of our mapping study, as follows:

\begin{itemize}
    \item \emph{Coverage}: it  estimates how largely a keyword has been investigated. This metric is defined as the sum of scores assigned to all the selected primary studies for each specific keyword. 
    \item \emph{Maturity}: it estimates how deeply a keyword has been investigated. It counts the number of papers that fully cover the keyword (i.e., papers having a 1 score for that keyword). 
\end{itemize}

In Fig.~\ref{fig:coverage_maturity}, we report \emph{Coverage} in light grey and \emph{Maturity} in dark-grey for all the keywords grouped by the four considered categories. Both metrics are drawn using bar charts that show the keywords on the y axis and the metric values on the x axis. As expected, the trend of the two metrics are closely related to the one in Figs.~\ref{fig:classification_research_area}~--~\ref{fig:classification_research_contribution}. However, since it is based on the evaluation we performed during the analysis of the primary studies, some specific conclusion can be drown.  

For most of the keywords, the two measures differ slightly, meaning that only a minority of the papers covering that keyword have shown a reduced maturity in dealing with it. It is expected for keywords like \emph{Performance engineering}, \emph{Performance analysis} or \emph{Performance evaluation} because they are general aspects considered in the context (for instance, a contribution can be focused on \emph{Self-adaptation} and providing in the meanwhile \emph{Performance analysis} - that is in this case evaluated with a score of 0,5). 

Interestingly, in Fig.~\ref{fig:coverage_maturity_domain}, \emph{Complex software systems} has a greater difference between coverage and maturity, meaning that several studies do not fully cover the domain (i.e., evaluated with a score of 0,5). While we tried to cover at least one domain for paper, this result means that there are several studies that do not properly belong to this specific domain, requiring dedicated solutions.
%
Going in Fig.~\ref{fig:coverage_maturity_contribution}, \emph{Tool support} has a greater difference between the two metrics, meaning that several studies do not provide an effective and mature tool support to the provided solution. 

On the other hand, some of the keywords (like \emph{Uncertainty}, \emph{Domain Specific Languages}, \emph{Data intensive systems}, \emph{Dev\-Ops}, and \emph{Agile}) have low values and small or none difference between coverage and maturity. This means that the low number of papers that contributed in these areas provided a mature and well-focused contribution. 

\textbf{\emph{Summarizing on RQ2:}}
The obtained results show that researchers in the performance software engineering area are interested in supporting modern {Complex software-intensive systems} with a growing employment of emerging practices, like continuous development and integration. The analysis confirms the trend discussed in Sect.~\ref{sec:results:rq1}. In fact, most primary studies significantly increased their maturity in this context in the last four years. On the other end, the architectural support for continuous software performance engineering research area is targeting new application domains, such as {Data-intensive systems}, {Embedded systems} and {Cyber-physical systems}. These application domains encompass specific target problems (e.g., {Uncertainty} and {Performance requirements}) and research contributions (e.g., {Domain specific languages}) are emerging to deal with them. 


==> _old_results-RQ3.tex <==
\subsection{Characteristics of approaches (RQ3)}
\noindent
The RQ3 is related to the characteristics of the approaches presented in the primary studies. The classification schema defines three main categories related to RQ3, namely Methodologies and techniques, Performance measures and indices, and Types of data. In the following, we first discuss about how the primary studies map these categories and  the variation of this mapping over the years. Then, we report on how the considered keywords combine in the existing contributions. 

\vspace{0.2cm}
\subsubsection{Characteristics of approaches} Figs.~\ref{fig:classification_techniques} -- ~\ref{fig:classification_data} depict the results of our mapping study for each of the above mentioned categories, by reporting the number of primary studies classified with respect to each keyword.

\underline{\emph{Methodologies and techniques.}} Fig.~\ref{fig:classification_techniques} shows the results for the Methodologies and techniques. Most approaches use well-assessed techniques like \emph{Performance models} and \emph{Performance analysis}. 
Other techniques related to the performance are largely used, such as \emph{Performance testing}, \emph{Performance model extraction}, and \emph{Performance prediction}. 

A few studies cover emerging techniques, such as \emph{Machine Learning} and \emph{Multi-objective optimization}, thus suggesting that future research shall further investigate the role of such  techniques in the context of continuous performance engineering. 
%
The figure also highlights that \emph{Model-drive engineering} techniques are not largely exploited in this field. Even the use of \emph{Model-based engineering} techniques does not emerge substantially, despite the primary studies focus on software architectures. This, combined to the observation that few studies consider \emph{Antipatterns and Pattern recognition}, suggests that model-driven and model-based methodologies can be further investigated and employed in the field of performance-targeted continuous software engineering.
%
Finally, \emph{Parametric Dependency} is still little studied opening to a further research direction in the future.



\begin{figure}[htpb]
    \centering
    \includegraphics[width=.95\linewidth]{figures/used_methodologies__techniques_0.5_to_1.pdf}
    \caption{Methodologies and techniques}%
    \label{fig:classification_techniques}
\end{figure}

\underline{\emph{Performance measures and indices.}} Figure~\ref{fig:classification_perf_measures} shows the results obtained in the category {Performance measures and indices}. The most used performance index is \emph{Response time}; this result is 
likely related to the system domain the studies belong to. In fact, the response time is a good performance estimator in contexts where users matter, such as (micro)services. Moreover, \emph{Response time}, \emph{Throughput}, and \emph{Utilization} are the three most used performance indices in performance analysis, while \emph{Network bandwidth} and \emph{Memory} are little considered. This is not surprising since they require a detailed description of the system under analysis and, hence, they are not suitable at the architectural description level.

\begin{figure}[htpb]
    \centering
    \includegraphics[width=.98\linewidth]{figures/used_performance_measure__indices_0.5_to_1.pdf}
    \caption{Performance measures and indices}%
    \label{fig:classification_perf_measures}
\end{figure}

\underline{\emph{Types of data.}}  Figure~\ref{fig:classification_data} depicts the {Types of data} exploited in our primary studies. Most of them are due to \emph{Monitored} and \emph{Runtime/Real-time} data. Although we are focused on performance analysis, few primary studies cover \emph{Workload} aspects, as well as  \emph{Requirements}, \emph{System models} and \emph{Data Analytics} are still little considered.


\begin{figure}[htpb]
    \centering
    \includegraphics[width=.95\linewidth]{figures/used_data_0.5_to_1.pdf}
    \caption{Types of data}%
    \label{fig:classification_data}
\end{figure}

\begin{comment}
\begin{figure}[htbp]
\centering
\hfil
\subfloat[\label{fig:coverage_in_time_methodologies_avg}Methodologies and techniques.]{
  \includegraphics[width=.95\linewidth]{figures/used_methodologies__techniques_coverage_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:coverage_in_time_measures_avg}Performance measures and indices.]{
  \includegraphics[width=.95\linewidth]{figures/used_performance_measure__indices_coverage_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:coverage_in_time_data_avg}Types of data.]{
  \includegraphics[width=.95\linewidth]{figures/used_data_coverage_in_time_avg.pdf}
}
\caption{\label{fig:rq3_coverage_in_time_avg}Average variation of coverage over the years (RQ3).}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}[htbp]
\centering
\hfil
\subfloat[\label{fig:maturity_in_time_methodologies_avg}Methodologies and techniques.]{
  \includegraphics[width=.95\linewidth]{figures/used_methodologies__techniques_maturity_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:maturity_in_time_measures_avg}Performance measures and indices.]{
  \includegraphics[width=.95\linewidth]{figures/used_performance_measure__indices_maturity_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:maturity_in_time_data_avg}Types of data.]{
  \includegraphics[width=.95\linewidth]{figures/used_data_maturity_in_time_avg.pdf}
}
\caption{\label{fig:rq3_maturity_in_time_avg}Average variation of maturity over the years (RQ3).}
\end{figure}
\end{comment}

\begin{figure}[htbp]
\centering
\hfil
\subfloat[\label{fig:mapping_in_time_methodologies_avg}Methodologies and techniques.]{
  \includegraphics[width=.95\linewidth]{figures/used_methodologies__techniques_mapping_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:mapping_in_time_measures_avg}Performance measures and indices.]{
  \includegraphics[width=.95\linewidth]{figures/used_performance_measure__indices_mapping_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:mapping_in_time_data_avg}Types of data.]{
  \includegraphics[width=.95\linewidth]{figures/used_data_mapping_in_time_avg.pdf}
}
\caption{\label{fig:rq3_mapping_in_time_avg}Average variation of mapping over the years (RQ3).}
\end{figure}


\underline{\emph{Mapping variation.}} 
In Figs.~\ref{fig:rq3_mapping_in_time_avg}, we reported the average variation of mapping over the years (i.e., before and after 2015). The obtained results confirm the trend discussed in Sec.~\ref{sec:results:rq1}, in fact most keywords significantly increased their values in the last four years. Going in more details, Fig.~\ref{fig:mapping_in_time_methodologies_avg} shows that \emph{Pattern recognition} and \emph{Performance analysis} are the unique techniques that decrease over the last four years, giving way other techniques to enhance. Among the other, the emerging techniques like \emph{Machine learning} and \emph{Model-driven techniques}, start to be employed after 2015. An interesting increasing trend can be observed for  \emph{Multi-objective optimization}, \emph{Parametric dependency}, \emph{Performance model extraction} and \emph{Performance prediction} in the contest of continuous software engineering. 
Figures~\ref{fig:mapping_in_time_measures_avg} and \ref{fig:mapping_in_time_data_avg} show increased values, meaning that recent approaches improved their maturity by better employing performance measures/indices and observed data. A special note deserves \emph{Network Bandwidth} that is the performance measure  recently studied in the contest of continuous software engineering, probably due to the cloud and (micro)services spread. 


\vspace{0.2cm}
\subsubsection{Clustering of characteristics}

As mentioned in Section~\ref{sec:method}, for each keyword, we assigned a score of $0$, $0.5$, or $1$ to each paper in our dataset of primary studies, depending on how much the paper is related to that keyword.
Therefore, after this evaluation, we obtained a vector to characterize each paper in a 52-dimensional space. 

In order to derive groups of closely related studies, we employed the \emph{hierarchical agglomerative clustering} (HAC) method~\cite{OmranES07}.
In our analysis, we used the \emph{Average Linkage} similarity metric, which is defined as the mean distance between elements of two candidate clusters, e.g. $A$ and $B$: $ {1 \over {|\mathcal{A}|\cdot|\mathcal{B}|}}\sum_{x \in \mathcal{A}}\sum_{ y \in \mathcal{B}} d(x,y) $.
In this similarity metric, we chose to compute the distance $d(x,y)$ between two papers using the cosine distance, which is the complement of the cosine of the angle between two vectors: $ 1 - \frac{u \cdot v} {||u||_2 ||v||_2} $.

\begin{figure}[htpb]
    \centering
    \includegraphics[width=.95\linewidth]{figures/hac.pdf}
    \caption{Dendrogram of the clustering performed on the dataset of primary studies.}%
    \label{fig:hac}
\end{figure}

Fig.~\ref{fig:hac} shows the dendrogram obtained by performing the clustering on the dataset.
In the figure, the $x$ axis reports the distance among clusters, whereas the $y$ axis reports the papers as they are numbered in the primary studies reference.
Even though the HAC technique builds the tree of all the clusters, ranging from the largest (the root) to the smallest (the leaves), it is possible to define a cut-off threshold in order to derive a desired number of clusters.
We have chosen the threshold which is represented by the dashed horizontal line.
In this way, we derived the 8 clusters that are drawn with different colors in the figure.
The choice of a threshold, while arbitrary, does not prevent a further inspection of a cluster by looking at the composition of its subtree.

Beside the very small clusters that are made of one or two papers, we are more interested in larger clusters which are colored in blue, red, green, and orange.
For these clusters we derived the subsets of the most common keywords:
\begin{itemize}[noitemsep]
    \item \emph{blue cluster}: Performance evaluation, Performance engineering, Monitored;
    \item \emph{red cluster}: Performance testing, Continuous software engineering, DevOps, Monitored;
    \item \emph{green cluster}: Performance engineering, Performance model, Requirements, Model-based engineering;
    \item \emph{orange cluster}: Self-adaptation.
\end{itemize}

The blue cluster, which contains 37 papers and therefore is by far the largest, is the one that more comprehensively represents the scope of our mapping study.
In fact, this cluster is characterized by approaches combining monitoring data and performance engineering to achieve performance validation during the development life cycle.
The red cluster brings together approaches integrating performance testing, based on monitoring information, into DevOps practices.
This may show a perceived increase in the relevance of performance testing in DevOps, and more specifically, in continuous software engineering.
Papers contained in the green cluster exploit performance modeling as the main technique for the verification of performance requirements.
In most cases, performance models, as employed in requirements validation, are augmented with information gathered from monitoring or are built entirely by extracting performance measures and inter-components interactions from runtime data.
Finally, the orange cluster contains papers that are set apart by a strong focus on self-adaptation.
This may suggest that, even when approaches rely on self-adaptation techniques as a mean of reacting to performance degradation at runtime, such methods are never part of a continuous engineering process.

From a closer look to the composition of the blue cluster, we can derive additional characteristics of interest. For instance, almost half of the papers makes intensive use of performance models, while only few of them provide even a preliminary tool support. Response time is undoubtedly the main measure of interest in the majority of papers, while memory usage, memory leaks, and resource allocation are rarely mentioned concerns. Performance requirements are also infrequently reported as target of the analysis, therefore considering only relative improvements of performance.

\textbf{\emph{Summarizing on RQ3:}}
The obtained results provide interesting insights. Our analysis shows that emerging techniques (e.g., Machine learning and Optimization) still lack of mature contributions in this mapping study context. Therefore, researchers shall explore them with the aim to support performance evaluation and prediction. Moreover, our results highlight that researchers shall exploit software models, also in terms of antipatterns combined with monitored data, to achieve more effective continuous engineering approaches embedding performance validation. 
Finally, the analysis pointed out how the traditional research on model-based performance engineering can be fruitfully enhanced by exploiting methodologies related to DevOps and Continuous monitoring/engineering practices.


==> figures.tex <==
\section*{Figures}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=.95\linewidth]{figures/new/research_area_horiz.pdf}
    \caption{Research area}
    \label{fig:research_area}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=.95\linewidth]{figures/new/domain__systems_domain_horiz.pdf}
    \caption{Domain}
    \label{fig:domain}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=.95\linewidth]{figures/new/target_problem_horiz.pdf}
    \caption{Target problem}
    \label{fig:target_problem}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=.95\linewidth]{figures/new/research_contribution_horiz.pdf}
    \caption{Research contribution}
    \label{fig:research_contribution}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=.95\linewidth]{figures/new/used_methodologies__techniques_horiz.pdf}
    \caption{Used methodologies / techniques}
    \label{fig:methodologies}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=.95\linewidth]{figures/new/used_performance_measure__indices_horiz.pdf}
    \caption{Used performance measures / indices}
    \label{fig:perf_measures_indices}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=.95\linewidth]{figures/new/used_data_horiz.pdf}
    \caption{Used data}
    \label{fig:data}
\end{figure}

\begin{figure}[htbp]
  \centering
  \subfloat[\label{fig:research_area_vert}Research area]{
    \includegraphics[width=10em]{figures/new/research_area_vert.pdf}
  }
  \subfloat[\label{fig:domain_vert}Domain]{
    \includegraphics[width=11em]{figures/new/domain__systems_domain_vert.pdf}
  }
  \subfloat[\label{fig:target_problem_vert}Target problem]{
    \includegraphics[width=8em]{figures/new/target_problem_vert.pdf}
  }
\end{figure}

\begin{figure}[htbp]
  \centering
  \subfloat[\label{fig:research_area_vert}Research contribution]{
    \includegraphics[width=11em]{figures/new/research_contribution_vert.pdf}
  }
  \subfloat[\label{fig:domain_vert}Used performance measures]{
    \includegraphics[width=10em]{figures/new/used_performance_measure__indices_vert.pdf}
  }
  \subfloat[\label{fig:research_area_vert}Used data]{
    \includegraphics[width=10em]{figures/new/used_data_vert.pdf}
  }
\end{figure}
\begin{figure}[htbp]
  \centering
  \subfloat[\label{fig:domain_vert}Used methodologies]{
    \includegraphics[width=.9\linewidth]{figures/new/used_methodologies__techniques_vert.pdf}
  }
\end{figure}

\begin{figure}[htbp]
  \centering
  \subfloat[\label{fig:bubble_perf_evaluation}Performance evaluation / assessment]{
    \includegraphics[width=.9\linewidth]{figures/new/bubble_performance_evaluation__assessment.pdf}
  }
  \hfill
  \subfloat[\label{fig:bubble_perf_req}Performance requirement]{
    \includegraphics[width=.9\linewidth]{figures/new/bubble_performance_requirement.pdf}
  }
\end{figure}
\begin{figure}\ContinuedFloat
  \subfloat[\label{fig:bubble_uncertainty}Uncertainty]{
    \includegraphics[width=.9\linewidth]{figures/new/bubble_uncertainty.pdf}
  }
  \hfill
  \subfloat[\label{fig:bubble_qos}Quality of service]{
    \includegraphics[width=.9\linewidth]{figures/new/bubble_quality_of_service.pdf}
  }
\end{figure}
\begin{figure}\ContinuedFloat
  \subfloat[\label{fig:bubble_resource_allocation}Resource allocation / deployment]{
    \includegraphics[width=.9\linewidth]{figures/new/bubble_resource_allocation__deployment.pdf}
  }
  \hfill
  \caption{\label{fig:bubble_target_problem}Considered target problems in combinations of research areas and domains.}
\end{figure}

\pagebreak


\begin{figure}[htbp]
    \centering
    \includegraphics[width=.98\linewidth]{figures/new/sankey_research_area_2_domain__systems_domain.pdf}
    \caption{Sankey diagram between research areas (left-hand side) and domains (right-hand side).}
    \label{fig:sankey_research_areas_domains}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=.98\linewidth]{figures/new/sankey_research_area_2_target_problem.pdf}
    \caption{Sankey diagram between research areas (left-hand side) and target problems (right-hand side).}
    \label{fig:sankey_research_areas_target_problems}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=.98\linewidth]{figures/new/sankey_research_area_2_research_contribution.pdf}
    \caption{Sankey diagram between research areas (left-hand side) and research contribution (right-hand side).}
    \label{fig:sankey_research_areas_research_contribution}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=.98\linewidth]{figures/new/sankey_research_area_2_used_methodologies__techniques.pdf}
    \caption{Sankey diagram between research areas (left-hand side) and used methodologies (right-hand side).}
    \label{fig:sankey_research_areas_used_methodologies}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=.98\linewidth]{figures/new/sankey_research_area_2_used_performance_measure__indices.pdf}
    \caption{Sankey diagram between research areas (left-hand side) and used performance measures (right-hand side).}
    \label{fig:sankey_research_areas_used_perf_measures}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=.98\linewidth]{figures/new/sankey_research_area_2_used_data.pdf}
    \caption{Sankey diagram between research areas (left-hand side) and used data (right-hand side).}
    \label{fig:sankey_research_areas_used_data}
\end{figure}

\pagebreak

\begin{figure}[htbp]
    \centering
    \subfloat[Research areas]{
        \includegraphics[width=.9\linewidth]{figures/new/radar_research_area.pdf}
    }
    \hfill
    \subfloat[Domain]{
        \includegraphics[width=.9\linewidth]{figures/new/radar_domain__systems_domain.pdf}
    }
\end{figure}
\begin{figure}[htbp]\ContinuedFloat
    \subfloat[Target problem]{
        \includegraphics[width=.9\linewidth]{figures/new/radar_target_problem.pdf}
    }
    \hfill
    \subfloat[Research contribution]{
        \includegraphics[width=.9\linewidth]{figures/new/radar_research_contribution.pdf}
    }
\end{figure}
\begin{figure}[htbp]\ContinuedFloat
    \subfloat[Used methodologies / techniques]{
        \includegraphics[width=.9\linewidth]{figures/new/radar_used_methodologies__techniques.pdf}
    }
    \hfill
    \subfloat[Used performance measures / indices]{
        \includegraphics[width=.9\linewidth]{figures/new/radar_used_performance_measure__indices.pdf}
    }
\end{figure}
\begin{figure}[htbp]\ContinuedFloat
    \subfloat[Used data]{
        \includegraphics[width=.9\linewidth]{figures/new/radar_used_data.pdf}
    }
\end{figure}

\pagebreak

==> figures/graphs.tex <==
\newpage

\begin{comment}
\begin{figure}[htbp]
\centering
\subfloat[\label{fig:coverage_in_time_research_area}Research area.]{
  \includegraphics[width=.95\linewidth]{figures/research_area_coverage_in_time.pdf}
}
\hfil
\subfloat[\label{fig:coverage_in_time_domain}Domain.]{
  \includegraphics[width=.95\linewidth]{figures/domain__systems_domain_coverage_in_time.pdf}
}
\hfil
\subfloat[\label{fig:coverage_in_time_target_problem}Target problem.]{
  \includegraphics[width=.95\linewidth]{figures/target_problem_coverage_in_time.pdf}
}
\hfil
\subfloat[\label{fig:coverage_in_time_contribution}Research contribution.]{
  \includegraphics[width=.95\linewidth]{figures/research_contribution_coverage_in_time.pdf}
}
\caption{\label{fig:coverage_in_time}Variation of coverage over the years (RQ2).}
\end{figure}

\begin{figure}[htbp]
\centering
\hfil
\subfloat[\label{fig:coverage_in_time_methodologies}Methodologies and techniques.]{
  \includegraphics[width=.95\linewidth]{figures/used_methodologies__techniques_coverage_in_time.pdf}
}
\hfil
\subfloat[\label{fig:coverage_in_time_measures}Performance measures and indices.]{
  \includegraphics[width=.95\linewidth]{figures/target_problem_coverage_in_time.pdf}
}
\hfil
\subfloat[\label{fig:coverage_in_time_data}Types of data.]{
  \includegraphics[width=.95\linewidth]{figures/research_contribution_coverage_in_time.pdf}
}
\caption{\label{fig:coverage_in_time}Variation of coverage over the years (RQ3).}
\end{figure}

\newpage

\begin{figure}[htbp]
\centering
\subfloat[\label{fig:maturity_in_time_research_area}Research area.]{
  \includegraphics[width=.95\linewidth]{figures/research_area_maturity_in_time.pdf}
}
\hfil
\subfloat[\label{fig:maturity_in_time_domain}Domain.]{
  \includegraphics[width=.95\linewidth]{figures/domain__systems_domain_maturity_in_time.pdf}
}
\hfil
\subfloat[\label{fig:maturity_in_time_target_problem}Target problem.]{
  \includegraphics[width=.95\linewidth]{figures/target_problem_maturity_in_time.pdf}
}
\hfil
\subfloat[\label{fig:maturity_in_time_contribution}Research contribution.]{
  \includegraphics[width=.95\linewidth]{figures/research_contribution_maturity_in_time.pdf}
}
\caption{\label{fig:maturity_in_time}Variation of maturity over the years (RQ2).}
\end{figure}

\begin{figure}[htbp]
\centering
\hfil
\subfloat[\label{fig:maturity_in_time_methodologies}Methodologies and techniques.]{
  \includegraphics[width=.95\linewidth]{figures/used_methodologies__techniques_maturity_in_time.pdf}
}
\hfil
\subfloat[\label{fig:maturity_in_time_measures}Performance measures and indices.]{
  \includegraphics[width=.95\linewidth]{figures/used_performance_measure__indices_maturity_in_time.pdf}
}
\hfil
\subfloat[\label{fig:maturity_in_time_data}Types of data.]{
  \includegraphics[width=.95\linewidth]{figures/used_data_coverage_in_time.pdf}
}
\caption{\label{fig:maturity_in_time}Variation of maturity over the years (RQ3).}
\end{figure}

\newpage

\begin{figure}[htbp]
\centering
\subfloat[\label{fig:coverage_in_time_research_area_avg}Research area.]{
  \includegraphics[width=.95\linewidth]{figures/research_area_coverage_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:coverage_in_time_domain_avg}Domain.]{
  \includegraphics[width=.95\linewidth]{figures/domain__systems_domain_coverage_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:coverage_in_time_target_problem_avg}Target problem.]{
  \includegraphics[width=.95\linewidth]{figures/target_problem_coverage_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:coverage_in_time_contribution_avg}Research contribution.]{
  \includegraphics[width=.95\linewidth]{figures/research_contribution_coverage_in_time_avg.pdf}
}
\caption{\label{fig:coverage_in_time_avg}Average variation of coverage over the years (RQ2).}
\end{figure}

\begin{figure}[htbp]
\centering
\hfil
\subfloat[\label{fig:coverage_in_time_methodologies_avg}Methodologies and techniques.]{
  \includegraphics[width=.95\linewidth]{figures/used_methodologies__techniques_coverage_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:coverage_in_time_measures_avg}Performance measures and indices.]{
  \includegraphics[width=.95\linewidth]{figures/used_performance_measure__indices_coverage_avg.pdf}
}
\hfil
\subfloat[\label{fig:coverage_in_time_contribution_avg}Types of data.]{
  \includegraphics[width=.95\linewidth]{figures/used_data_coverage_in_time_avg.pdf}
}
\caption{\label{fig:coverage_in_time_avg}Average variation of coverage over the years (RQ3).}
\end{figure}

\newpage
\end{comment}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





\begin{figure}[htbp]
\centering
\subfloat[\label{fig:maturity_in_time_research_area_avg}Research area.]{
  \includegraphics[width=.95\linewidth]{figures/research_area_maturity_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:maturity_in_time_domain_avg}Domain.]{
  \includegraphics[width=.95\linewidth]{figures/domain__systems_domain_maturity_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:maturity_in_time_target_problem_avg}Target problem.]{
  \includegraphics[width=.95\linewidth]{figures/target_problem_maturity_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:maturity_in_time_contribution_avg}Research contribution.]{
  \includegraphics[width=.95\linewidth]{figures/research_contribution_maturity_in_time_avg.pdf}
}
\caption{\label{fig:rq2_maturity_in_time_avg}Average variation of maturity over the years (RQ2).}
\end{figure}

\begin{figure}[htbp]
\centering
\hfil
\subfloat[\label{fig:maturity_in_time_methodologies_avg}Methodologies and techniques.]{
  \includegraphics[width=.95\linewidth]{figures/used_methodologies__techniques_maturity_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:maturity_in_time_measures_avg}Performance measures and indices.]{
  \includegraphics[width=.95\linewidth]{figures/used_performance_measure__indices_maturity_in_time_avg.pdf}
}
\hfil
\subfloat[\label{fig:maturity_in_time_data_avg}Types of data.]{
  \includegraphics[width=.95\linewidth]{figures/used_data_maturity_in_time_avg.pdf}
}
\caption{\label{fig:rq3_maturity_in_time_avg}Average variation of maturity over the years (RQ3).}
\end{figure}

==> future-short.tex <==
\subsection{Implication for future research}\label{sec:future}
\noindent
In this section we discuss the implications of this study and challenges for future research.

\subsubsection{Towards a culture of quality in CSE}
\noindent
The results obtained suggest an interest in a culture of quality, indicating that analysis and verification occur early in the CSE pipeline (as for testing in DevOps), making it easier to discover and fix defects with a collaborative approach to product improvement. In order to bring up the quality characteristics of software (architecture) and its continuous improvement (and re-architecting), QoS analysis must become an integrated activity in the entire lifecycle of software development lifecycle, which requires continuous exposure of quality characteristics exposed to analysis. 

As discussed earlier, most of the selected studies focused on a few of the performance properties. However, there is a need to strengthen the support for various properties in both performance and, in general, software quality during the continuous engineering of the system. 
%
Some challenging quality aspects to consider are: verification of correctness properties, such as architectural mismatches, 
evaluation of the architectural runtime models with respect to fidelity and usefulness for human inspection, extending the scalability by considering influencing factors such as variation in the complexity of user behavior in experiments, supporting
state management and resource provisioning mechanism, and
introducing time consumption for memory allocation and release operations to increase the prediction quality of the model.
Similarly, other QoS properties, such as the reliability, consistency, safety and security, and availability can be modeled and analyzed in a CSE framework.


\subsubsection{Performance engineering benefits in DevOps}
\noindent
DevOps is gaining widespread adoption in industry. However, its principles of rapid changes, development automation, and fast feedback loop (often relying on dynamic cloud environments) conflict with the complexity of the current performance engineering approaches.
Thus, performance engineering frameworks should be improved for adoption in rapidly changing systems. The structures and behaviors of the modern systems changes frequently and requires continuous relearning of the failure models in order to retain the prediction quality. 

Moreover, these systems are characterized by a continuous stream of available data. Performance models should be built periodically, incrementally, or even continuously, and be triggered by changes to components in the monitored environment. Models can be quickly rebuilt once a potential problem is detected using only the most recent data only, and then used to compare with previous model results.

\subsubsection{Data-driven methods and Machine Learning}
Performance and load tests produce a large amount of data that can be difficult to analyze. Data-driven methods provide powerful insights into optimizing performance, building new features, and preventing problems with services, especially in distributed (enterprise) applications, in-memory databases, and big data systems.

Despite developments  in modern software engineering technology, there is no established methodology for systematically employing performance engineering and data-driven engineering in continuous development.

In addition, performance evaluation based on machine learning can become an integral part of the continuous engineering process. The performance model must learn autonomously and improve itself during system operation in a production environment.


\subsubsection{Continuous controlling system uncertainty}
\noindent
As discussed in Sections \ref{sec:results:rq2} and \ref{sec:results:rq4}, uncertainty has been addressed marginally in the papers selected in this study. However, both in academia and industry, significant attention is paid to the contexts characterized by a high degree of uncertainty. To reduce uncertainty and obtain feedback on products/software as soon as possible, it is important to test assumptions and hypotheses in short cycles \cite{CSE}.

Continuous monitoring and frequent re-assessment and re-architecting are necessary to reduce the uncertainty in CSE and DevOps. An efficient analysis method can be used to propagate the eﬀect of uncertain parameters in software systems and calculate the robustness of the performance indices, thereby enhancing the flexibility in addressing uncertainty.


\subsubsection{Integration and abstraction}
\noindent
A recurring issue is the need to integrate methods and tools into the continuous and DevOps pipelines. Hence, it is necessary to design and develop performance engineering approaches that can be integrated with other tools and methods used in the context of this study. 

Continuous monitoring is a fundamental process in CSE. In the context of implications for future research, further investigation on adaptive monitoring and analysis infrastructure that can automatically update the system and performance/quality models is needed. 

External capabilities can be integrated using approaches to represents systems as black-box components by integrating black-box monitoring techniques, or creating resource profiles describing specific enterprise applications (using standard measurement solutions), instead of relying on a custom solution to collect the required data. This can be improved by supporting the collection of arbitrary information on the status of the monitored application, which requires the system integration of the corresponding type on a dynamic basis.

Using a higher abstraction level can help reduce the integration efforts. Future research can target the development of a model-based framework that considers the definition of (domain-specific) languages and automation mechanisms to ensure, by design, the potential for the monitoring, analysis, testing, and simulation in CSE. As discussed above, machine learning-supported and data-driven approaches can be used to (continuously) learn and tune the models. 

\subsubsection{Implications for practitioners and researchers}
\noindent
Practitioners can benefit from the presented results to understand how software performance engineering and software architectural can support practices in CSE and DevOps. Moreover, they can benefit from the classification of methodologies applicable to architectural support for performance engineering in the context of continuous software development.  

Researchers can benefit from our results to understand research trends and research gaps, and to better focus on their future work. In particular, the software performance community can leverage this work to understand whether their approaches are applicable in a CSE/DevOps context. Moreover, this study helps them define the requirements that drive the development of their tools to increase the chances of industrial adoption. In contrast, researchers in the field of CSE/DevOps can identify which methodologies and techniques can help improve software performance at some stage in the development cycle.


\smallskip
\noindent\fbox{%
    \parbox{\linewidth}{%
    \noindent
    %\smallskip
    \emph{Main findings:}
    \begin{itemize}[leftmargin=*]
        \item There is a growing interest for a culture of quality, where quality properties are continuously exposed to analysis and verification during the software development life-cycle;
        \item The complexity of the current performance engineering approaches should  improve their suitability for the DevOps principles of rapid changes, development automation, and fast feedback loop;
        \item There is a need for an established methodology for the systematically employment of performance engineering and machine learning/data-driven engineering in continuous development;
        \item Continuous monitoring and frequent re-assessment and re-architecting are necessary to reduce uncertainty in CSE and DevOps;
        \item Using higher abstraction level (i.e. by means of a model-based framework or (domain-specific) languages and automation mechanisms) can help in reducing the effort of integrating heterogeneous methods and components in systems. 
    \end{itemize}
    
    }%
}

==> results-RQ1-short.tex <==
\section{What research areas and target systems have been investigated (RQ$_1$)}
\label{sec:results:rq1}

\noindent
The  topic considered combines several aspects, as we discussed in Section~\ref{sec:related}, which may attract interest from different disciplines and for different scopes of research. To  provide an overview of this research topic, we describe the research areas focused on providing solutions and the target systems for which solutions have been developed.

%\subsection{Research areas}
%\noindent
Figure~\ref{fig:research_area} depicts the principal \underline{\textbf{research areas}} that are focus areas of the selected papers (each study may contribute to more than one area). The bar chart in the figure compares the identified research areas with respect to the number of papers \footnote{Although our topic is characterized by the dimensions shown in this figure, the fact that the selected papers contribute to these specific fields of research is not obvious. For instance, a paper may just use a specific performance evaluation technique without contributing in that area.} For each research area, we stacked two different bars to combine both the \emph{fully} and \emph{partially investigated} areas (as described in Section~\ref{sec:process-extraction}). 

As expected, the selected papers mainly focus on the areas of \emph{software performance engineering} and \emph{software architecture}, which is in agreement with the information on publication venues obtained in the publication trends.
%

Many studies have contributed to \emph{continuous software engineering} that considered at least one of the continuous dimensions introduced in Section \ref{sec:related}, 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=.95\linewidth]{figures/new/research_area_horiz.pdf}
    \caption{Research areas - results}
    \label{fig:research_area}
\end{figure}

Significant attention has been paid to the continuous monitoring of data to realize continuous development, delivery, and integration, which improves system performance at the level of SA. As the monitored data enable performance analysis, continuous monitoring represents a fundamental capability to provide CSE. In general, the results confirm that in the areas of SA and SP, CSE is an emerging topic that is progressively gaining the interest of researchers and practitioners. 
%
Existing conferences and systematic reviews on {DevOps} suggest that software engineering researchers have a strong interest in this topic. Despite this, only a few papers focus on {DevOps}, underling an interesting gap to be addressed by the research community. However, the limited number of articles on {agile} is an expected result. Even as a precursor to DevOps, agile development is more code-focused and produces less documentation (e.g., software/design models), disabling SA-based SPE.


\begin{figure}[htbp]
    \centering
    \includegraphics[width=.95\linewidth]{figures/new/domain__systems_domain_horiz.pdf}
    \caption{Target systems - results}
    \label{fig:domain}
\end{figure}


Although a large number of selected papers have been fully identified as contributors to the CSE field, the number of papers that partially investigate this area has increased. Beyond that, several selected papers have not been placed within the context of CSE or DevOps, which can be attributed to the fact that these papers do not explicitly place themselves in these areas, even if they actually oﬀer solutions that cover several aspects of an iterative development process, wherein updates are made continuously. However, this confirms that this emerging theme is gaining ground.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Target systems}
%\noindent

\revnew{Figure~\ref{fig:domain} describes the specific type of  \underline{\textbf{target systems}} (as case studies) by selected papers. These keywords are not meant to be mutually exclusive, in that a system could be, for example, at the same time a distributed and real-time one. We have basically identified, in each paper, the main characteristics of systems to which the paper approach/solutions have been (or can be potentially) applied, where they have been unambiguously identified.}




\emph{Component-based software} and \emph{software intensive} systems have been most investigated. These targets are characterized by the existence of different components, services, or subsystems. These can be independent of each other (e.g., microservices) or have strong dependencies and relationships amongst themselves and with the environment, as in many complex systems. However, in both cases, the presence of heterogeneous components makes it necessary to integrate these activities into continuous development and maintenance (e.g., DevOps). The component-based development paradigm is based on the concept of reuse within distinct components (e.g., services), enabling integration. Once integrated and implemented, these components must enter a continuous dimension, that is, to know and analyze the behavior after the integration and not only of the single component; therefore, they are also important in the context of performance.

Next, the results show the targets of \emph{cloud} and \emph{distributed systems}, characterized by the technology stack and infrastructure complexity. Cloud nodes may attain performance orders of magnitude worse than other nodes \cite{armbrust09}. For instance, if during the hosting of a mission-critical service or a scientific application, performance variability and availability become a concern, cloud monitoring is required to continuously measure and assess the infrastructure or application behavior (in terms of performance, reliability, power usage, and security) to adapt the system to changes or to apply corrective measures. Generally, we can observe that in open systems characterized by uncontrolled requests, continuous engineering, which supports their integration and evolution, is fundamental to identifying the occurrence of further problems not observed before.

Finally, we note that more recent and innovative targets are not yet widely investigated. For instance, in the case of \emph{data intensive} systems, the massive use of big data and machine learning requires efficient management of resources, performance, and security.

\smallskip
\noindent\fbox{
    \parbox{\linewidth}{
    \noindent
    \emph{Main findings:}
    \begin{itemize}[leftmargin=*]
        \item Significant attention is paid to continuous monitoring of data, which represents a fundamental capability to provide CSE;
        \item CSE and DevOps are gaining ground: most studies offer solutions covering several aspects of the iterative development process where updates are made continuously;
        \item Software intensive systems, especially when component-based, are the most investigated ones: their heterogeneous components require the integration of their activities in a continuous development and maintenance;
        \item More recent and innovative targets, such as cloud and data intensive systems, have not been widely investigated.
    \end{itemize}
    }
}


==> results-RQ2-short.tex <==
\section{What and how performance problems have been addressed (RQ$_2$)}
\label{sec:results:rq2}
\noindent
We classified the \SelectedFullPapers selected papers by considering the research problems addressed by them (we divided the target problems into five categories), and their research contributions (we identified seven diﬀerent types of contributions). In particular, the selected papers were thematically associated with at least one target problem and at least one research contribution based on their research directions and scope. We provide a detailed overview of the performance problems that have been addressed and illustrate them with  exemplary papers.

%\subsection{Research problems}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=.95\linewidth]{figures/new/target_problem_horiz.pdf}
    \caption{Research problems - results}
    \label{fig:target_problem}
\end{figure}

\noindent
Figure~\ref{fig:target_problem} presents the problems targeted by the selected papers (\underline{\textbf{research problems}}). 
The results obtained confirm that most of the selected papers are aimed at solving performance evaluation and assessment problems. This is a relevant goal in the development of modern systems, where increasingly agile paradigms require that performance analyses be in a continuous dimension to be effective.

Part of the selected papers aims to provide \emph{QoS}, where the target is to satisfy different requirements/properties for the overall quality of the system, including guaranteeing a certain level of performance.

Managing the \emph{uncertainty} of the system behavior is an emergent topic (papers addressing this issue are recent publications), and it is cross-cutting to the target problems previously mentioned. Although having the complete model of the system represents the ideal situation, in practice, only partial and limited measures are available. Consequently, specialized performance analysis or prediction techniques must work with uncertain knowledge. The proposed studies and their discussions on the diﬀerent types of uncertainty highlight relevant issues and offer new research ideas.




%%%%%%%%%%%%%%%%%%







%\subsection{Research contributions}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=.95\linewidth]{figures/new/research_contribution_horiz.pdf}
    \caption{Research contributions - results}
    \label{fig:research_contribution}
\end{figure}

%\noindent
Figure~\ref{fig:research_contribution} describes the principal \underline{\textbf{research contributions}}. From our analysis, we can state that most of the studies contribute to the continuous performance assessment of the system with \emph{performance analysis, performance modelling, and performance prediction} approaches. Most of the approaches use performance evaluation to achieve the desired QoS objectives in software systems.

More than half of the research problems considered were addressed using the support of dedicated \emph{tools} or CSE \emph{frameworks} and were well partitioned between performance prediction, performance analysis, and performance modelling. This is an interesting result, as in the context of this study, the quality and performance requirements demand the support of continuous engineering frameworks or dedicated tools.

Other research problems were dedicated to \emph{self-adaptation} approaches and, to a lesser extent, \emph{domain-specific languages}. The latter result shows that few studies have exploited abstraction for continuous performance control, although they consider large heterogeneous runtime data. Raising the level of abstraction of the specification would favour increased automation and interoperability.
%%%%%%%%%%%%%%%%%





\smallskip
\noindent\fbox{%
    \parbox{\linewidth}{%
    \noindent
    %\smallskip
    \emph{Main findings:}
    \begin{itemize}[leftmargin=*]
        \item Performance prediction, performance analysis and performance modelling have been further explored in order to offer adequate support in continuous developing;
        \item A relevant number of self-adaptation approaches have been proposed to ensure the quality of services (including performance); 
        \item Quality and performance requirements demand for the support of continuous engineering frameworks or dedicated tools.
    \end{itemize}
    }%
}




==> results-RQ3-short.tex <==
\section{What instruments have been adopted (RQ$_3$)}
\label{sec:results:rq3}
\noindent
Performance analysis can be conducted by adopting multiple techniques with different output-targeted metrics and with the support of different types of input data. In this section, we aim to identify the instruments that are adopted more often in the context of the study.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/new/rq3.pdf}
    \caption{Data, methodologies/techniques, measures/indices - results}
    \label{fig:rq3}
\end{figure}


Figure~\ref{fig:rq3}(a) reports the input \underline{\textbf{data}}. In regard to CSE, a system is continuously monitored to feed performance indices back into a performance model that supports predictive analyses. 

A total of $61$ and $32$ papers (of \SelectedFullPapers) used \emph{runtime/monitored} and \emph{performance model} as input data, respectively. Lesser number of papers consider the performance model as the input data because performance models have only been integrated in the last few years of software engineering processes.
Whereas runtime performance assessment and fixing have long been considered as common practices.
Majority of the papers that used monitored data also proposed a continuous approach to monitoring performance features and then used them mainly for analysis and prediction.

A significant number of papers considered the \emph{software model} as an input to the process. This is likely due to the different notations that are usually adopted for representing software models, preventing an automated full integration in the performance assessment task. 

The results here also provide evidence that \emph{data analytics} has not yet been largely considered in this domain. However, interest in data analytics has grown over time; thus, data analytics is expected to become a primary source of inputs in the next few years.


Figure~\ref{fig:rq3}(b) presents the \underline{\textbf{methodologies/techniques}} used in the selected papers. As expected, the majority of papers are focused on with \emph{performance modeling} and \emph{performance analysis}. It is necessary to build and analyze models to address the performance issues early in the lifecycle. \emph{Model based software engineering} and \emph{model driven engineering} techniques were also widely considered, as they did not restrict the adoption of models to the performance domain.  A considerable number of papers deal with \emph{performance model extraction} and \emph{performance testing} techniques which were typically adopted when studying performance issues on existing running software systems. Finally, it is observed that although in the last few years the adoption of \emph{machine learning} and \emph{multi-objective optimization} techniques has spread in diverse fields in the context of CSE, they are still marginally considered.

It is observed that this occurs despite the fact that \emph{performance modeling} is fully investigated. In certain contexts, extensive performance analysis can be difficult owing to the lack of system measurements and parameter values. Hence, in such cases, performance modeling can be fully investigated, but the analysis remains marginal among the contributions of the papers. 


Figure~\ref{fig:rq3}(c) shows the targeted output \underline{\textbf{measures/indices}}. The three typical performance indices, namely, \emph{response time}, \emph{utilization}, and \emph{throughput}, are the most widely targeted ones in the considered papers. Although, on one hand, this can be seen as an expected outcome, on the other hand it is somehow surprising that \emph{memory} and \emph{network bandwidth} have been significantly less studied in this context. These two measures may play crucial roles in the performance assessment of modern heterogeneous distributed software systems. Hence this result evidences a lack of investigation in this direction. 




\smallskip
\noindent\fbox{%
    \parbox{\linewidth}{%
    \noindent
    %\smallskip
    \emph{Main findings:}
    \begin{itemize}[leftmargin=*]
        \item Approaches of performance modeling and analysis techniques that take as input monitored data and produce response time and utilization indices as output are widely used methodologies. Requirements and data analytics rarely enter the process to target memory and network bandwidth;
        \item Even if machine learning and multi-objective optimization techniques are being increasingly studied, they are still marginally considered in the context of CSE;
        \item Model-based  and model-driven techniques are widely considered, as they do not restrict the adoption of models to the performance domain, but in several cases, software models are also considered.
    \end{itemize}
    }%
}

==> results-RQ4-short.tex <==
\section{Current research gaps and future directions (RQ$_4$)}
\label{sec:results:rq4}

\noindent
In this section, we aim at detecting potential research gaps by visualizing the number of papers that lie at the intersection of research areas and target systems for each keyword of interest. In the following section, we discuss our findings in the categories of keywords:  \emph{target problems}, \emph{research contributions}, \emph{used methodologies and techniques}, \emph{used performance measures and indices}, and \emph{input data}. To represent our results, we developed bubble plots, as described in Section \ref{sec:method}. Moreover, we discuss the implications for future research based on the research gaps analyzed and future directions described in the selected papers.


\subsection{Research problems and contributions}\label{sec:results:rq4:target}
\noindent
Figures \ref{fig:bubble_target_problem_performance_evaluation__assessment} and \ref{fig:bubble_target_problem_uncertainty} show the bubble plots for the \emph{Performance evaluation} and \emph{Uncertainty} research problems, respectively.
The plots present a very different situation.
Many studies have targeted the problem of performance evaluation, especially in certain areas, and few papers have considered the uncertainty in general. A reason for this may be attributed to the fact that uncertainty has emerged only recently as a distinct concern in software engineering and its inclusion in continuous engineering practices is still very limited.

\begin{figure*}[]
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/new/bubble_target_problem_performance_evaluation__assessment}
\caption{Number of papers investigating the keyword \emph{performance evaluation (target problem)} at the intersection of research areas and target systems.}
\label{fig:bubble_target_problem_performance_evaluation__assessment}
\end{minipage}%
  \hfill
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/new/bubble_target_problem_uncertainty}
\caption{Number of papers investigating the keyword \emph{uncertainty (target problem)} at the intersection of research areas and target systems.}
\label{fig:bubble_target_problem_uncertainty}
\end{minipage}
%\caption{Selected Papers by Types and by Years}
% \label{fig:papertypeandyear}
\end{figure*}


% \begin{figure}[htbp]
% \centering
% \includegraphics[width=.9\linewidth]{figures/new/bubble_target_problem_performance_evaluation__assessment}
% \caption{Number of papers investigating the keyword \emph{performance evaluation (target problem)} at the intersection of research areas and target systems.}
% \label{fig:bubble_target_problem_performance_evaluation__assessment}
% \end{figure}

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=.9\linewidth]{figures/new/bubble_target_problem_uncertainty}
% \caption{Number of papers investigating the keyword \emph{uncertainty (target problem)} at the intersection of research areas and target systems.}
% \label{fig:bubble_target_problem_uncertainty}
% \end{figure}


In contrast, because the general problem of performance evaluation is specifically targeted by our study, a greater number of papers are expected to consider it from Figure~\ref{fig:bubble_target_problem_performance_evaluation__assessment}, it is evident that certain research areas (continuous monitoring, DevOps, and agile) never intersect with certain target systems (real-time, embedded and CPS) when pursuing performance evaluation.
This could simply be due to the scarce adoption of DevOps and agile practices in these systems. 

A further gap appears in the area of the development of software intensive systems, even if it is continuously evolving  owing to the adoption of  new technologies, such as cloud computing, IoT, and artificial intelligence; Continuous engineering and DevOps can benefit from new performance engineering solutions to achieve more pervasive software (for example in smart cities, smart manufacturing, and smart mobility).




Among several research contributions identified, we reported the plots for \emph{continuous engineering framework} (Figure~\ref{fig:bubble_research_contribution_continuous_engineering_framework}) and \emph{performance prediction} (Figure~\ref{fig:bubble_research_contribution_performance_prediction_approach}) as we considered them to be relevant for the purposes of our study.
In Figure~\ref{fig:bubble_research_contribution_continuous_engineering_framework}, we observe that most of the papers proposing a novel continuous engineering framework are gathered in the lower half of the plot.
The target systems for which most of these frameworks are designed are CBS/SOA/Microservices, software intensive systems, and distributed systems.
Predictably, CSE is the most targeted research area in this field.
However, continuous engineering frameworks are rarely or never proposed in real-time and embedded systems.

\begin{figure*}[]
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/new/bubble_research_contribution_continuous_engineering_framework}
\caption{Number of papers investigating the keyword \emph{continuous engineering framework (research contribution)} at the intersection of research areas and target systems.}
\label{fig:bubble_research_contribution_continuous_engineering_framework}
\end{minipage}%
  \hfill
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/new/bubble_research_contribution_performance_prediction_approach}
\caption{Number of papers investigating the keyword \emph{performance prediction (research contribution)} at the intersection of research areas and target systems.}
\label{fig:bubble_research_contribution_performance_prediction_approach}
\end{minipage}
%\caption{Selected Papers by Types and by Years}
% \label{fig:papertypeandyear}
\end{figure*}


% \begin{figure}[htbp]
% \centering
% \includegraphics[width=.9\linewidth]{figures/new/bubble_research_contribution_continuous_engineering_framework}
% \caption{Number of papers investigating the keyword \emph{continuous engineering framework (research contribution)} at the intersection of research areas and target systems.}
% \label{fig:bubble_research_contribution_continuous_engineering_framework}
% \end{figure}

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=.9\linewidth]{figures/new/bubble_research_contribution_performance_prediction_approach}
% \caption{Number of papers investigating the keyword \emph{performance prediction (research contribution)} at the intersection of research areas and target systems.}
% \label{fig:bubble_research_contribution_performance_prediction_approach}
% \end{figure}


Figure~\ref{fig:bubble_research_contribution_performance_prediction_approach} shows that only a few papers proposed performance prediction approaches in embedded, real-time, and data-intensive systems.
In addition, only three papers appear to focus on both DevOps and agile.
This may represent a research gap about to be filled in the next few years because approaches based on artificial intelligence and machine learning, such as those in the AIOps \cite{AIOPS} field, are rapidly emerging as a new way of modeling and predicting performance that can be more easily integrated with current DevOps practices.




\subsection{Data, methodologies/techniques, and measures/indices}
\noindent
The types of data that are used as input to the approaches play a significant role in establishing the situations in which an approach can be applied and the type of information required to initiate the process. \emph{Workload} (Figure~\ref{fig:bubble_used_data_workload}) and \emph{requirements} (Figure~\ref{fig:bubble_used_data_requirements}) are the types of data, consideration of which appears to be related to the specific target system.
For instance, while the workload is often considered in the \emph{cloud}, \emph{distributed}, and \emph{CBS/SOA/microservices} systems, it is rarely considered in \emph{embedded}, \emph{real-time}, and \emph{data intensive} systems. The lack of consideration of workload in embedded and real-time systems is expected, whereas in data intensive systems it presents a research opportunity. When considering the use of requirements, we are presented with a different situation. From the number of papers in the bubble plot, it appears that \emph{DevOps} and \emph{agile} do not put much emphasis on the requirements when assessing the performance; this is unexpected because they consider the specification of requirements in their processes. 

\begin{figure*}[]
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/new/bubble_used_data_workload}
\caption{Input data - Workload}
\label{fig:bubble_used_data_workload}
\end{minipage}%
  \hfill
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/new/bubble_used_data_requirements}
\caption{Input data - Requirements}
\label{fig:bubble_used_data_requirements}
\end{minipage}
%\caption{Selected Papers by Types and by Years}
% \label{fig:papertypeandyear}
\end{figure*}



% \begin{figure}[htbp]
% \centering
% \includegraphics[width=.9\linewidth]{figures/new/bubble_used_data_workload}
% \caption{Input data - Workload}
% \label{fig:bubble_used_data_workload}
% \end{figure}

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=.9\linewidth]{figures/new/bubble_used_data_requirements}
% \caption{Input data - Requirements}
% \label{fig:bubble_used_data_requirements}
% \end{figure}



In addition, the \emph{software intensive} and \emph{CBS/SOA/micorservices} systems often consider the requirements as the starting point for the development of performance engineering approaches.

The methodologies and techniques that are employed in the approaches of our study represent a compelling source of information for discovering the current research interests and gaps. For instance, when examining the use of performance models (Figure~\ref{fig:bubble_used_methodologies__techniques_performance_model}), it is clear that the DevOps and agile research areas lag behind the other areas in terms of the number of papers. 

\begin{figure*}[]
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/new/bubble_used_methodologies__techniques_performance_modeling}
\caption{Methodologies / techniques - Performance model}
\label{fig:bubble_used_methodologies__techniques_performance_model}
\end{minipage}%
  \hfill
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/new/bubble_used_methodologies__techniques_performance_testing__load_testing__benchmarking}
\caption{Methodologies / techniques - Performance testing / Load Testing / Benchmarking}
\label{fig:bubble_used_methodologies__techniques_performance_testing__load_testing__benchmarking}
\end{minipage}
%\caption{Selected Papers by Types and by Years}
% \label{fig:papertypeandyear}
\end{figure*}


% \begin{figure}[]
% \centering
% \includegraphics[width=.9\linewidth]{figures/new/bubble_used_methodologies__techniques_performance_modeling}
% \caption{Methodologies / techniques - Performance model}
% \label{fig:bubble_used_methodologies__techniques_performance_model}
% \end{figure}

% \begin{figure}[]
% \centering
% \includegraphics[width=.9\linewidth]{figures/new/bubble_used_methodologies__techniques_performance_testing__load_testing__benchmarking}
% \caption{Methodologies / techniques - Performance testing / Load Testing / Benchmarking}
% \label{fig:bubble_used_methodologies__techniques_performance_testing__load_testing__benchmarking}
% \end{figure}




\begin{figure*}[]
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/new/bubble_used_methodologies__techniques_performance_model_generation__extraction}
\caption{Methodologies / techniques - Performance model generation / extraction}
\label{fig:bubble_used_methodologies__techniques_performance_model_generation__extraction}
\end{minipage}%
  \hfill
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/new/bubble_used_methodologies__techniques_simulation}
\caption{Methodologies / techniques - Simulation}
\label{fig:bubble_used_methodologies__techniques_simulation}
\end{minipage}
%\caption{Selected Papers by Types and by Years}
% \label{fig:papertypeandyear}
\end{figure*}




% \begin{figure}[]
% \centering
% \includegraphics[width=.9\linewidth]{figures/new/bubble_used_methodologies__techniques_performance_model_generation__extraction}
% \caption{Methodologies / techniques - Performance model generation / extraction}
% \label{fig:bubble_used_methodologies__techniques_performance_model_generation__extraction}
% \end{figure}

% \begin{figure}[]
% \centering
% \includegraphics[width=.9\linewidth]{figures/new/bubble_used_methodologies__techniques_simulation}
% \caption{Methodologies / techniques - Simulation}
% \label{fig:bubble_used_methodologies__techniques_simulation}
% \end{figure}

A different picture is presented using performance testing, as shown in Figure~\ref{fig:bubble_used_methodologies__techniques_performance_testing__load_testing__benchmarking}. In this case, while all the research areas are almost equally represented, a lack of focus on the adoption of performance testing, load testing, and benchmarking is evident in the real-time and embedded systems, as the number of papers contributing to above-mentioned aspects in the real-time embedded systems are 0 and 3, respectively. Generation or extraction of a performance model (Figure~\ref{fig:bubble_used_methodologies__techniques_performance_model_generation__extraction}) is a special use case in the adoption of performance models. Therefore, unsurprisingly, we can still count a few papers in the DevOps and agile research areas, whereas distributed and microservice systems seem to rely the most on the automated generation of performance models.
Finally, in regard to the use of simulation (shown in Figure~\ref{fig:bubble_used_methodologies__techniques_simulation}), we observed that, in contrast to other methodologies, simulation has been employed in several papers for real-time and embedded systems. In addition, DevOps and agile appear to be less represented than in other research areas.

When investigating the performance measures and indices that were targeted as outputs in the selected papers, we observed two radically different situations in the number of papers that considered the keywords \emph{response time} (Figure~\ref{fig:bubble_used_performance_measure__indices_response_time}) and \emph{memory/memory leaks} (Figure~\ref{fig:bubble_used_performance_measure__indices_memory__memory_leaks}).
In software performance engineering, response time and memory are among the primary measures of interest as they are usually employed to assess the quality of service and operating costs, respectively. Nonetheless, memory is rarely considered in the papers selected for this study. Even more interesting is the fact that \emph{DevOps} and \emph{agile} seem to not consider memory at all in any target system. We expect memory use to become critical as ML and data-intensive systems continue to increase.
In contrast, response time is considered more often in general and in particular in the  domains of \emph{distributed systems}, \emph{software intensive systems}, and \emph{CBS/SOA/imcroservices}. 
This paints a picture in which performance measures that impact the quality of service are the foremost concern in research related to CSE, thus resulting in a substantial gap in the investigation of issues related to memory usage and how these can affect the cost of providing a service.


\begin{figure*}[]
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/new/bubble_used_performance_measure__indices_response_time}
\caption{Output measures / indices - Response time}
\label{fig:bubble_used_performance_measure__indices_response_time}
\end{minipage}%
  \hfill
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/new/bubble_used_performance_measure__indices_memory__memory_leaks}
\caption{Output measures / indices - Memory / Memory Leaks}
\label{fig:bubble_used_performance_measure__indices_memory__memory_leaks}
\end{minipage}
%\caption{Selected Papers by Types and by Years}
% \label{fig:papertypeandyear}
\end{figure*}



% \begin{figure}[]
% \centering
% \includegraphics[width=.9\linewidth]{figures/new/bubble_used_performance_measure__indices_response_time}
% \caption{Output measures / indices - Response time}
% \label{fig:bubble_used_performance_measure__indices_response_time}
% \end{figure}

% \begin{figure}[]
% \centering
% \includegraphics[width=.9\linewidth]{figures/new/bubble_used_performance_measure__indices_memory__memory_leaks}
% \caption{Output measures / indices - Memory / Memory Leaks}
% \label{fig:bubble_used_performance_measure__indices_memory__memory_leaks}
% \end{figure}








\smallskip
\noindent\fbox{%
    \parbox{\linewidth}{%
    \noindent
    %\smallskip
    \emph{Main findings:}
    \begin{itemize}[leftmargin=*]
        \item Although performance evaluation is a very well-established research topic, the conjunction with the latest trends in the software industry, such as agile and DevOps, is overdue.
        \item Researchers have started to study software performance under uncertainty. The research area has not yet been sufficiently investigated but may possess great growing potential.
        \item There is no evidence of the experience of companies in conducting performance analytics on cloud systems.
    \end{itemize}
    }%
}



==> table_1.tex <==

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=1\textwidth]{figures/scheme}
    \caption{\label{fig:scheme}Classification scheme}
    \label{fig:classificationScheme}
\end{figure*}


\begin{table}[]
\centering
\footnotesize
\begin{tabular}{|l|l|l|}
\hline
\textbf{RQ} & \textbf{Data}            & \textbf{Metrics}                                                                                                                                            \\ \hline
                                                  & Research area     & \#Fully investigated topics (F)                                                                                                                    \\ \cline{2-3} 
                                                  & Research domain   & \#Partially investigated topics (P)                                                                                                                \\ \cline{2-3} 
\multirow{-3}{*}{RQ1}                             &                   & \#investigated topics (P ; F)                                                                                                                      \\ \hline
                                                  & Target Problems   & \begin{tabular}[c]{@{}l@{}}\#Main target  problem/contributions (M)\end{tabular}                                                                 \\ \cline{2-3} 
                                                  & Contributions     & \begin{tabular}[c]{@{}l@{}}\#Secondary target  problem/contributions (S)\end{tabular}                                                            \\ \cline{2-3} 
\multirow{-3}{*}{RQ2}                             &                   & \begin{tabular}[c]{@{}l@{}}\#Main or Secondary target \\ problem/contributions (M, S)\end{tabular}                                                 \\ \hline
                                                  & Methodologies     & \#Fully evaluated  indices/data/methods (F)                                                             \\ \cline{2-3} 
                                                  & Indices (output)  & \#Partially evaluated indices/data/methods (P)                                                         \\ \cline{2-3} 
\multirow{-3}{*}{RQ3}                             & Used Data (input) & \#Fully or Partially evaluated indices/data/methods (F, P)                                           \\ \hline
RQ4                                               &                   & \begin{tabular}[c]{@{}l@{}}??? \textbackslash{}DT\{da inserire una volta capito \\ quali metriche o grafici sono \\ rappresentativi\}\end{tabular} \\ \hline
RQ5                                               &                   & \begin{tabular}[c]{@{}l@{}}??? \textbackslash{}DT\{da inserire una volta capito \\ quali metriche o grafici sono \\ rappresentativi\}\end{tabular} \\ \hline
\end{tabular}%

\caption{Data Extraction, and Metrics adopted for the analysis.} 
\label{tab:DataExtraction} 
\end{table}
